Fault Tolerance by Construction

A key challenge in fault-tolerant quantum computing is synthesising and optimising circuits in a noisy environment, as traditional techniques often fail to account for the effect of noise on circuits. In this work, we propose and numerically verify a framework for designing fault-tolerant quantum circuits that are correct by construction. The framework starts with idealised specifications of fault-tolerant gadgets and refines them using provably sound basic transformations. To reason about manipulating circuits while preserving their error correction properties, we define fault equivalence; two circuits are considered fault-equivalent if all undetectable faults on one circuit have a corresponding fault on the other. This guarantees that the effect of undetectable faults on both circuits is the same. We argue that fault equivalence is a concept that is already implicitly present in the literature. Many problems, such as state preparation and syndrome extraction, can be naturally expressed as finding an implementable circuit that is fault-equivalent to an idealized specification. To utilize fault equivalence in a computationally tractable manner, we adapt the ZX calculus, a diagrammatic language for quantum computing. We restrict its rewrite system to not only preserve the underlying linear map but also fault equivalence, i.e. the circuit's behaviour under noise. Enabled by our framework, we verify, optimise, and synthesise new and efficient circuits for syndrome extraction and cat state preparation. We confirm the improved performance of our optimised circuits in simulation. We anticipate that fault equivalence can capture and unify different approaches in fault-tolerant quantum computing, paving the way for an end-to-end circuit compilation framework.

==> sections/old/02-prerequisites.tex <==
\section{ZX Calculus}
The ZX calculus~\parencite{coeckeInteractingQuantumObservables2008} is a graphical formalism for quantum computation and is particularly well suited for reasoning about stabilizer circuits and Clifford operations.
The calculus has two key features: it allows any quantum circuit to be represented using ZX diagrams, and it provides rewrite rules for transforming these diagrams.
We provide a brief introduction to the Clifford fragment of ZX calculus~\parencite{backensZXcalculusComplete2014}; for a comprehensive overview of the complete calculus, readers are referred to \textcite{vandeweteringZXcalculusWorkingQuantum2020}.

\subsection{ZX Diagrams}

A ZX diagram is a graphical representation of a linear map, composed of interconnected nodes with parameters and colours.
Nodes are referred to as \enquote{spiders}, of which there are two types represented by their colour, green Z-spiders and red X-spiders (hence ZX).\footnote{For readers viewing in black and white or with limited colour vision, green spiders appear lightly shaded and red spiders appear darkly shaded.}
Each spider carries a phase parameter $\alpha \in [0, 2\pi)$ and has an arbitrary number of \enquote{legs} or connections, which represent its input/output qubit ports.
\begin{align*}
  \textit{Z-spider:} \qquad
  \tikzfig{02-prelims/ZX/z-spider}
  \quad &\coloneqq \quad
  \ket{0}^{\otimes n}\! \bra{0}^{\otimes m} + e^{i k\frac{\pi}{2}} \ket{1}^{\otimes n}\! \bra{1}^{\otimes m}\\[8pt]
  \textit{X-spider:} \qquad
  \tikzfig{02-prelims/ZX/x-spider}
  \quad &\coloneqq \quad
  \ket{+}^{\otimes n}\! \bra{+}^{\otimes m} + e^{i k\frac{\pi}{2}} \ket{-}^{\otimes n}\! \bra{-}^{\otimes m}
\end{align*}
In the Clifford fragment of the ZX calculus, phases are restricted to multiples of $\frac{\pi}{2}$.
By convention, if the phase parameter is not explicitly annotated on a spider, it defaults to $0$.
Additionally, we introduce the yellow \emph{Hadamard box}, $\tikzfig{02-prelims/ZX/hadamard-box}$, which represents the Hadamard gate.

Formally, we define ZX diagrams as follows:
\begin{definition}[ZX diagram]
  A ZX diagram $D$ is defined as a graph $G = (V, E)$ with phases for vertices $\alpha \colon V \to \{0, \frac{\pi}{2}, \pi, \frac{3\pi}{2}\}$ and vertex types $t \colon V \to \{Z, X, B\text{(oundary)}\}$.
  Here, boundary nodes indicate inputs and outputs.
  For a ZX diagram $D$, we denote the linear map it represents by $\interp{D}$, and we call the $\interp{\cdot}$ the \emph{interpretation} function.
  \label{def:zx-diagram}
\end{definition}

\begin{definition}[Boundary and internal edges]
  Edges connected to an input or output are called \emph{input edges} and \emph{output edges}, respectively.
  Collectively, these are referred to as \emph{boundary edges}, while all other edges are called \emph{internal edges}.
\end{definition}

\paragraph{Mapping Clifford Circuits to ZX Diagrams}

To rigorously analyze quantum circuits using graphical methods, we first formalize the objects involved: quantum circuits and the process of mapping them to ZX diagrams.

\begin{definition}[Quantum Circuit]
  \label{def:quantum-circuit}
  A \emph{quantum circuit} $C$ over a gate set $\mathcal{G}$ is specified by a sequence of gates $(g_1, g_2, \dots, g_L)$.
  Each gate $g_k \in \mathcal{G}$ acts on a specified set of input and output wires.
  The circuit $C$ corresponds to the composed linear operator $\interp{C} = g_L \circ g_{L-1} \circ \dots \circ g_1$.
\end{definition}

Mapping such a circuit to a ZX diagram involves representing gates as diagrams and composing them according to the circuit structure, ensuring the resulting diagram represents the same operation.

\begin{definition}[ZX Mapping]
  \label{def:zx-mapping}
  Let $\mathcal{C}(\mathcal{G})$ be a set of quantum circuits over a gate set $\mathcal{G}$, and $\mathcal{ZX}$ be the set of ZX diagrams.
  A \emph{ZX Mapping} is a function $\mathcal{M}: \mathcal{C}(\mathcal{G}) \to \mathcal{ZX}$ defined as follows:
  \begin{enumerate}
    \item $\mathcal{M}$ assigns a specific ZX diagram $\mathcal{M}(g) \in \mathcal{ZX}$ to each gate $g \in \mathcal{G}$ such that $\interp{g} = \interp{\mathcal{M}(g)}$.
    \item For any circuit $C = g_L \circ \dots \circ g_1$, the mapping is extended compositionally via:
    \[
      \mathcal{M}(C) = \mathcal{M}(g_L) \circ \mathcal{M}(g_{L-1}) \circ \dots \circ \mathcal{M}(g_1)
    \]
  \end{enumerate}
\end{definition}

While different choices for the gate assignments $\mathcal{M}(g)$ in step 1 result in different ZX mappings, for most gates there is a conventional ZX counterpart.
Each fundamental Clifford gate has a standard ZX equivalent: for instance, the S gate corresponds to a green Z-spider with phase $\frac{\pi}{2}$, while the Pauli X gate is represented by a red X-spider with phase $\pi$.
\autoref{fig:mappings} illustrates quantum states, single-qubit Clifford gates, and two-qubit operations mapped into ZX under the standard mapping.
\begin{figure}[htb]
  \begin{minipage}{.30\textwidth}
    \begin{align*}
      \ket{0}
      \quad
      &\longmapsto \quad
      \tikzfig{02-prelims/ZX/x-state-zero} \\[8pt]
      \ket{+}
      \quad &\longmapsto \quad
      \tikzfig{02-prelims/ZX/z-state-zero} \\[8pt]
      \tikzfig{02-prelims/QC/not}
      \quad &\longmapsto \quad
      \tikzfig{02-prelims/ZX/not} \\[8pt]
      \tikzfig{02-prelims/QC/y}
      \quad &\longmapsto \quad
      \tikzfig{02-prelims/ZX/y} \\[8pt]
      \tikzfig{02-prelims/QC/s}
      \quad &\longmapsto \quad
      \tikzfig{02-prelims/ZX/s} \\[8pt]
    \end{align*}
  \end{minipage}
  \begin{minipage}{.35\textwidth}
    \begin{align*}
      \tikzfig{02-prelims/QC/cnot}
      \quad \longmapsto& \quad
      \tikzfig{02-prelims/ZX/cnot} \\[8pt]
      \tikzfig{02-prelims/QC/cz}
      \quad \longmapsto& \quad
      \tikzfig{02-prelims/ZX/cz} \\[8pt]
      \tikzfig{02-prelims/QC/zz-parity-check}
      \quad \longmapsto& \quad
      \tikzfig{02-prelims/ZX/ParityCheck} \\
    \end{align*}
  \end{minipage}
  \begin{minipage}{.35\textwidth}
    \begin{align*}
      \tikzfig{02-prelims/QC/zzzz-parity-check}
      \quad &\longmapsto \quad
      \tikzfig{02-prelims/ZX/ParityCheck-4} \\
    \end{align*}
  \end{minipage}
  \caption{Mapping quantum circuits representing common states and operations to ZX diagrams.}
  \label{fig:mappings}
\end{figure}
Notice that for single-qubit gates, the spider's phase directly encodes the rotation on the Bloch sphere, offering an intuitive picture of the gate's geometric effect.
For a concrete example of how a quantum circuit is mapped to a ZX diagram, see \autoref{fig:example-circuit}.

\begin{figure}[hbt]
  \[
    \tikzfig{02-prelims/QC/steane-encoder}
    \quad \overset{(a)}{\longmapsto} \quad
    \tikzfig{02-prelims/ZX/steane-encoder}
    \quad \overset{(b)}{=} \quad
    \tikzfig{02-prelims/ZX/steane-encoder-nf}
  \]
  \caption{(a) The encoder of the Steane code as a quantum circuit and its equivalent representation as a ZX diagram. (b) Equating two ZX-diagrams to reveal deeper structural properties. For every CSS code, a similar diagram can be acquired which tells us the stabilizers of the code.}
  \label{fig:example-circuit}
\end{figure}

\subsection{Rewrite Rules}

Beyond representing quantum circuits, the distinguishing feature of the ZX calculus lies in its set of graphical rewrite rules.
These rewrites allow ZX diagrams to be transformed into equivalent diagrams (i.e.\@ representing the same linear map) by applying local transformations within a larger diagram.
This enables the manipulation, simplification, and verification of quantum computations directly in the graphical language.

First and foremost, a fundamental rewrite of the ZX calculus, often assumed implicitly, is that \emph{Only Connectivity Matters} (\emph{OCM}).
This principle allows us to rearrange spiders and bend their legs, provided the overall connectivity and the positions of inputs/outputs of the diagram are preserved.
For example, the following diagrams are all considered equivalent under OCM:
\[
  \tikzfig{02-prelims/OCM}
\]

The core rewrite rules of the ZX calculus are referred to as axioms, from which complex transformations can be derived.
\autoref{fig:axioms} illustrates a set of axioms known to be complete (up to global scalars) for the Clifford fragment of the ZX calculus~\parencite{backensZXcalculusComplete2014}.
Completeness means that any equivalence between Clifford operations can be proven solely by applying these graphical rules.
This gives the calculus a deductive power equal to matrix algebra, but within an intuitive graphical framework.

\begin{figure}[htb]
  \[
    \tikzfig{02-prelims/axioms}
  \]
  \caption{A complete set of axioms for the Clifford fragment of the ZX calculus. Equalities shown hold up to scalars.}
  \label{fig:axioms}
\end{figure}

\paragraph{Interpreting Key Rewrite Rules}

The utility of the ZX calculus becomes clearer when we examine how individual rewrite rules encode familiar quantum concepts or aid in specific procedures.
We now illustrate this with three examples relevant to our discussion.

Consider the spider fusion rule \TextFusion.
It enables us to merge connected spiders of the same colour and their phases are added up.
This rule graphically represents the commutation of operators that are diagonal in the same basis and enables the verification commutation relations between quantum gates.
For example, it can be easily verified graphically that the S gate commutes with the CZ gate:
\[
  \tikzfig{02-prelims/commutation}
\]

Another common rule is the pi-copy rule \TextPiCommute which describes how $\pi$ phased spiders propagate through spiders of the opposite colour.
This encodes the fundamental algebraic structure relating the X and Z bases, manifesting well-known commutation and anticommutation relations.
For example, we can show how the $YZ$ propagates through a CNOT gate:
\[
  \tikzfig{02-prelims/pauli-propagation}
\]

An additional area where the ZX excels is circuit synthesis, often leading to novel circuit designs.
Previous works include phase gadget synthesis~\parencite{cowtanPhaseGadget2020} and floqetification~\parencite{rodatzFloquetifyingStabiliser2024}.
As a basic example, we can use ZX to synthesize a circuit representing the $ZZZZ$ stabilizer measurement.
We start by translating the $ZZZZ$ measurement to ZX according to \autoref{fig:mappings}, and transforming it so that only circuit-like operations remain:
\begin{gather}
  \tag{$r_{naive}$}\label{r-naive}\refstepcounter{equation}
  \tikzfig{02-prelims/ZZZZ}
\end{gather}

Besides the above examples, the ZX calculus is generally useful for visualizing, understanding, and verifying existing concepts, and often serves as a unifying language connecting ideas from different domains~\parencite{bombinUnifyingFlavorsFault2024}.
For example, CSS codes can be represented particularly elegantly within ZX~\parencite{kissingerPhasefreeZXDiagrams2022}, while other concepts like code morphisms~\parencite{huangGraphicalCSSCode2023} and lattice surgery~\parencite{debeaudrapZXCalculus2020} can be intuitively understood using the ZX calculus.

\subsection{Extensions for Scalability}

%\begin{definition}[ZX diagram]
%  We define a ZX diagram $D$ as a graph $G = (V, E_n, E_i)$ with vertices $V$ and two types of edges; normal edges $E_n$ where faults can occur and idealized, fault-free edges $E_i$.
%  Each vertex has a phases $\alpha \colon V \to \{0, \frac{\pi}{2}, \pi, \frac{3\pi}{2}\}$ and vertex type $t \colon V \to \{Z, X, B\text{(oundary)}\}$ where boundary nodes are used to indicate inputs and outputs.
%  For a ZX diagram $D$, we denote the linear map it represents by $\interp{D}$.
%  This function $\interp{\cdot}$ that maps diagrams to linear maps is called the \emph{interpretation} function.
%\end{definition}

%We define two different edge types; noisy and noise-free.
%The distinction will become relevant in the following section, where we define noise on ZX diagrams.
%Noise-free edges are an idealized mathematical tool that will help us reason about quantum circuits.
%Diagrammatically, we differentiate the edge types by drawing noisy edges in black and noise-free edges in purple.

While standard ZX diagrams provide a powerful framework, their representation can become visually complex for large quantum systems, and expressing hierarchical structures or abstract processes requires further conventions.
To address these points and enhance readability, we adopt two notational extensions.

First, borrowing elements from the scalable ZX calculus~\parencite{caretteSZXCalculusScalable2019}, we use scalable wires to compactly represent multiple qubits:
\[
  \tikzfig{02-prelims/scalable-zx}
\]

Second, to manage abstraction and focus on the high-level role of components, we represent sub-diagrams or specific processes using boxes, a technique common in diagrammatic reasoning and Categorical Quantum Mechanics~\parencite{coeckePicturingQuantum2017}.
For instance, we may define the following processes:
\[
  \tikzfig{02-prelims/boxes}
\]
By convention, triangles denote state preparations and measurements, while trapezoids represent encoders or decoders.
When the concrete content of the boxes becomes relevant, we can revert to the corresponding ZX diagrams.

%When drawing a box with purple\BOLDI{blue and maybe remove boundaries} boundaries, we mean that all internal nosy edges in the box are replaced by noise-free edges:
%\[\tikzfig{02-prelims/noise-removal}\]

\subsection{Pauli Webs}

Pauli webs~\parencite{bombinUnifyingFlavorsFault2024} are a decoration of the Clifford ZX calculus that track how Paulis propagate through a diagram.
They do so by highlighting edges in red and/or green according to a set of simple rules:
\begin{definition}[Pauli web]
  Given a ZX diagram $D$, a Pauli web $\{(e_1, t_1), \dots, (e_n, t_n)\}$ is a set of pairs containing an edge $e_i \in D$ and the corresponding type $t_i \in \{Z, X\}$, such that:
  \begin{itemize}
    \item a spider with $0$ or $\pi$ phase can have:
    \begin{itemize}
      \item an even number of legs highlighted in its own colour, \textbf{and/or}
      \item all or none of its legs highlighted in the opposite colour
    \end{itemize}
    \item a spider with $\pm \frac{\pi}{2}$ phase can have \textbf{either}:
    \begin{itemize}
      \item an even number of legs highlighted in its own colour and no legs highlighted in the opposite colour, \textbf{or}
      \item an odd number of legs highlighted in its own colour and all legs highlighted in the opposite colour
    \end{itemize}
    \item a Hadamard box must have the same number of green and red legs
  \end{itemize}
  \label{def:pauli-web}
\end{definition}
\noindent
These local rules ensure that the web at each spider is consistent with Paulis it commutes and anticommutes with, thus guaranteeing the global validity of the web.
\autoref{fig:pauli-web-examples} shows an example of each possible single-spider case from \autoref{def:pauli-web}, while examples of Pauli-web on a larger diagrams are shown in \autoref{example:detecting-region}.

\begin{figure}[htb]
  \[
    \tikzfig{02-prelims/ZX/pauli-web-examples}
  \]
  \caption{Example Pauli webs on a single spider.}
  \label{fig:pauli-web-examples}
\end{figure}

Pauli webs are in formal correspondence with the stabilizers and logicals of the diagram~\parencite{rodatzFloquetifyingStabiliser2024}.
Following \textcite{townsend-teagueFloquetifyingColourCode2023}, we classify them as detecting regions, stabilizing Pauli webs, or logical Pauli webs, depending on the types of edges they cover.

\begin{definition}[Detecting region]
  A detecting region is a Pauli web that highlights no boundary edges.
\end{definition}

\begin{definition}[(Co)stabilizing Pauli web]
  A Pauli web that highlights no input edges is a stabilizing Pauli web and, one that highlights no output edges is a co-stabilizing Pauli web.
\end{definition}

\begin{definition}[Logical Pauli webs]
  A (non-trivial) logical Pauli web is a Pauli web that is not a stabilizing or a co-stabilizing Pauli web, or the product of such webs.
\end{definition}

For syndrome extraction circuits of quantum error correction codes, stabilizing Pauli webs and logical Pauli webs are in bijective correspondence with the stabilisers and logicals of the corresponding code.   

\begin{example}
  \[
    \tikzfig{02-prelims/ZX/pauli-web-types-example}
  \]
  \label{example:detecting-region}
\end{example}

\begin{proposition}
  \label{thm:detecting-region}
  Let $D$ be a ZX diagram with a detecting Pauli web $P$.
  Let $n$ be the number of spiders in $D$ that anticommute with $P$ and $m$ the number of edges highlighted as $Y$.
  Then, if $n + m$ is odd, $\interp{D} = 0$.
\end{proposition}
\begin{proof}
  We can fire all the spiders in $D$ according to $P$ without changing the interpretation of the diagram.
  For each edge, we push one of the newly introduced spiders, adding a global phase of $(-1)^n$ due to the $n$ anticommuting operators.
  Now, every edge has two Pauli spiders of the same type, which cancel each other out.
  Since in our framework a $Y$ edge corresponds to the product of an $X$ and a $Z$ edge, a global $(-1)^m$ scalar is introduced.
  Therefore, we have derived that $\interp{D} = (-1)^{n+m} \interp{D}$.
  If $n + m$ is odd, then $\interp{D} = -\interp{D}$, implying that $\interp{D} = 0$.
\end{proof}


==> sections/old/03-errors.tex <==
\section{Errors on Diagrams}

Designing fault-tolerant circuits requires understanding how quantum circuits behave under noise.
While they are typically analyzed using established noise models, such as phenomenological or circuit noise, these do not naturally translate to ZX diagrams.
This section addresses this by introducing a noise model tailored to ZX diagrams and developing a framework for translating from quantum circuits while preserving behaviour under a given noise model.

%The main goal of designing fault-tolerant circuits is to find circuits that behave well under noise.
%For this, we have to formalize what we mean by behaviour under noise.
%As we are eventually interested in synthesizing new circuits, we are primarily concerned with ZX diagrams.
%Therefore, we define a noise model on ZX diagrams: edge flip.
%The edge flip noise model is purposefully kept simple, considering Pauli errors on edges of ZX diagrams.

%We still want to relate this noise models to noise models on quantum circuits, such as phenomenological noise, CSS noise and circuit noise.
%However, to make the manipulation of ZX diagrams independent of the choice of noise model, we make this connection not by changing our noise model.
%Instead, we change how we translate from quantum circuits to ZX diagrams.
%For this, we make use of the observation that different ZX diagrams can represent the same quantum circuit, however, display different behaviour under noise.
%Using this, we define the notion of a ZX diagram being \textit{fault-accounting} for a quantum circuit.
%
%Using all of these insights, we finally define when we consider two ZX diagrams to be equivalent under noise.
%As we are working in an error correction context, we only care about the effect of undetectable errors on the respective ZX diagrams, saying that two diagrams $D_1$ and $D_2$ are equivalent under noise if all undetectable errors on $D_1$ have a corresponding error on $D_2$ with the same effect and vice versa.

\subsection{Noisy and Idealized Edges}

Let us extend the definition of standard ZX diagrams from \autoref{def:zx-diagram} by incorporating two types of edges: noisy and idealized.
Idealized, noise-free edges serve as a mathematical tool that will help us reason about quantum circuit synthesis and FTQC, while noisy edges are the locations where faults can occur.

\begin{definition}[ZX diagram with noisy and idealized edges]
  Let $D$ be a ZX diagram defined by a graph $G = (V, E)$ with associated vertex types and phases.
  A \emph{ZX diagram with noisy and idealized edges} is given by $D$ with an additional edge colouring $f \colon E \to \{N, I\}$, where $N$ denotes \emph{noisy} and $I$ denotes \emph{idealized}.
  For convenience, we define the set of noisy edges as $E_n \coloneqq \{e \in E\ |\ f(e) = N\}$ and the set of idealized edges as $E_i \coloneqq \{e \in E\ |\ f(e) = I\}$.
  This paper differentiates the edge types by drawing noisy edges in black and idealized edges in purple.
\end{definition}

\subsection{Edge Flips}

We define a noise model inherent to ZX diagrams, where elementary errors can occur on the edges connecting nodes in a ZX diagram.
Unlike phenomenological or circuit-level models often tied to specific qubits, gate operations, or physical time evolution, this edge-based approach provides a structural and time-independent perspective on noise localization within the abstract graphical representation.

\begin{definition}[Edge flip]
  Given a ZX diagram $D$ with noisy and idealized edges, an \emph{edge flip} in $D$ is a tuple $(e, t)$ where
  \begin{itemize}
    \item $e \in E_n$ is a noisy edge in $D$ and
    \item $t \in \{X, Y, Z\}$ is the error type.
  \end{itemize}
  We write $D + (e, t)$ to denote the diagram with the Pauli corresponding to $t$ applied to the edge $e$.
\end{definition}

\begin{figure}[htb]
  \[
    \tikzfig{03-errors/error-example-base}\ +\ ((3,4), X)
    \qquad = \qquad
    \tikzfig{03-errors/edge-flip-example} \qquad = \qquad
    \tikzfig{03-errors/edge-flip-example-ocm}
  \]
  \caption{Applying the edge flip $((3,\ 4),\ X)$ to a ZX diagram (with annotated vertices).}
  \label{fig:example-edge-flip}
\end{figure}

\autoref{fig:example-edge-flip} demonstrates the effect of the edge flip $((3, 4), X)$.
The initial diagram (left) is transformed into the middle diagram by the flip.
This middle diagram is equivalent under OCM to the rightmost diagram, yet they suggest different physical interpretations: a single qubit error versus an error internal to a CNOT gate structure, respectively.
It contrasts with circuit noise models where errors are typically tied to fixed components (qubits, specific gates).
Therefore, edge flips are best understood as abstract modifications within the ZX calculus, rather than errors with a predetermined physical meaning.

We now define a \emph{fault} as a composite error representing a potential noise event comprising one or more atomic edge flips.
It is formally defined as follows:
\begin{definition}[Fault]
  Given a ZX diagram $D$, a \emph{fault} $\mathcal{F}$ is a set of edge flips $\mathcal{F} = \{(e_1, t_1), \dots, (e_n, t_n)\}$ where each $(e_i, t_i)$ is an edge flip in $D$.
  \begin{itemize}
    \item The \emph{weight} of a fault $wt(\mathcal{F})$ is the number of unique edges effected: $wt(\mathcal{F}) = |\{ e \mid (e, t) \in \mathcal{F} \}|$.
    \item We denote the diagram resulting from applying the fault as $D + \mathcal{F}$.
    \item Two faults $\mathcal{F}_1, \mathcal{F}_2$ are \emph{equivalent} if they lead to the same interpretation: $\interp{D + \mathcal{F}_1} = \interp{D + \mathcal{F}_2}$.
    \item A fault $\mathcal{F}$ is \emph{trivial} if it does not change the diagram's interpretation: $\interp{D + \mathcal{F}} = \interp{D}$.
  \end{itemize}
\end{definition}

%As a useful mathematical tool, we additionally introduce a new type of edges for ZX diagrams: idealized, fault-free edges.
%Faults on a ZX diagram are, by definition, not allowed to contain edge flips of fault-free edges.
%While such edges obviously do not exist on quantum computers, fault-free edges are a very useful tool to reason about ZX diagrams under noise.
%We draw fault-free edges in purple:
%\[
%  \tikzfig{02-prelims/noise-removal}
%\]
%Drawing a box with purple edges represents the underlying diagram with all its internal edges replaced by an idealized one.

\subsection{Fault-Accounting ZX Diagrams}

We have seen that quantum circuits can be mapped to ZX diagrams; however, mappings do not consider noise models.
We seek a representation where circuit-level noise have direct, simple counterparts within the mapped diagram.
We introduce a formal property for ZX diagrams that achieve this strong correspondence, specifically requiring that relevant circuit faults can be mapped to single edge flips in the diagram.

\begin{definition}[Fault accounting diagram]
  \label{def:fault-accounting}
  A ZX diagram $D$ is \emph{fault-accounting} for a quantum circuit $C$ under some noise model, if
  \begin{enumerate}
    \item $\interp{D} = \interp{C}$ and
    \item for all faults $f$ in $C$, there exists an edge flip $(e, t)$ in $D$ such that $\interp{C + f} = \interp{D + (e, t)}$.
  \end{enumerate}
\end{definition}

\paragraph{Fault-Accounting Representations for Phenomenological Noise}

Recall from \autoref{def:zx-mapping} that mapping circuits to ZX diagrams is a compositional process where each gate is replaced by its ZX representation, and these diagrams are connected according to the circuit's topology.
Given such a mapping, we can relate our edge-flip based noise model to other noise models.

\begin{proposition}
  Let $N_{phenom}$ be the phenomenological noise model consisting only of (i) single Pauli errors occurring on qubit wires between gate applications and (ii) classical bit flips on measurement outcomes.
  Given any quantum circuit $C$ and ZX mapping $\mathcal{M}$, the mapped ZX diagram $\mathcal{M}(C)$ is fault-accounting for $C$ under phenomenological noise $N_{phenom}$.
\end{proposition}
\begin{proof}
  Any Pauli error on a qubit corresponds to an edge flip on the corresponding edge in the ZX diagram.
  Classical flips of measurement outcomes can similarly be modeled by edge flips;
  for destructive measurement, they are equivalent to a qubit flip and for Pauli measurements, they correspond to flips on the edge before the measurement.
\end{proof}

\paragraph{Fault-Accounting Representations for Circuit Noise}

While the standard ZX Mapping is fault-accounting under phenomenological noise, it does not generally produce fault-accounting diagrams for multi-qubit gates when considering circuit noise models that include multi-qubit Pauli errors.
A key example is the CNOT gate: its standard representation $\mathcal{M}_{std}(CNOT)$ fails to provide single edge flips corresponding to all two-qubit Pauli errors that might follow the gate;
see \autoref{fig:cnot-unaccounted}, illustrating the unaccounted faults.

\begin{figure}[htb]
  \[
    \tikzfig{03-errors/fault-accounting/cnot-faults-unaccounted}
  \]
  \caption{Pauli faults (XY, XZ, YY, YZ) that are unacconted for as a single edge-flip in the standard ZX representation of the CNOT gate.}
  \label{fig:cnot-unaccounted}
\end{figure}

Fault-accounting representations for such gates can, however, be constructed by incorporating \emph{fault gadgets} into the diagram structure.
A fault gadget $G$ is a ZX diagram that represents the identity operation, $\interp{G} = I$, but has an internal edge where an edge flips yields a desired multi-qubit Pauli error.
The gadget shown in \autoref{fig:fault-gadget}, for instance, maps a single internal $Z$ flip to a $Z \otimes Z$ fault on its two output edges.
By conjugating with appropriate Clifford gates, gadgets can be designed to generate other Pauli errors.

\begin{figure}[htb]
  \[\tikzfig{03-errors/zz-fault-gadget-in-action}\]
  \caption{The ZZ fault gadget and its correctness}
  \label{fig:fault-gadget}
\end{figure}

Using this technique, a fault-accounting diagram for the CNOT gate, denoted $D'_{CNOT}$, is constructed by composing the standard diagram $\mathcal{M}_{std}(CNOT)$ with the necessary set of (conjugated) fault gadgets, one for each Pauli error not already accounted for by $\mathcal{M}_{std}(CNOT)$:
\[
  D'_{CNOT} = (G_{YZ} \circ G_{YY} \circ G_{XZ} \circ G_{XY}) \circ \mathcal{M}_{std}(CNOT)
\]


\begin{proposition}
  \label{prop:CNOT-fault-accounting}
  Let $N_{Pauli_2}$ be the noise model where any two-qubit Pauli error may occur immediately after the CNOT gate.
  Then the following ZX diagram is fault-accounting for the CNOT-gate under $N_{Pauli_2}$:
  \[
    \tikzfig{03-errors/fault-accounting/CNOT} \qquad \overset{fault-accounting}{\mapsto} \qquad \tikzfig{03-errors/fault-accounting/fault-accounting-cnot}
  \]
\end{proposition}
\begin{proof}
  By \autoref{def:fault-accounting}, we have to show that (1) $D'_{CNOT}$ represents the CNOT gate and that (2) it accounts for Pauli faults via single edge flips.
  \begin{enumerate}
    \item Since each fault gadget $G_f$ interprets as the identity, $\interp{D'_{CNOT}} = \interp{\mathcal{M}_{std}(CNOT)} = \interp{CNOT}$.
    \item By construction, for every non-trivial two-qubit Pauli fault $f \coloneqq P_1 \otimes P_2$, there exists a single edge flip $(e_f, t_f)$ in $D'_{CNOT}$ such that $\interp{D'_{CNOT} + (e_f, t_f)} = \interp{(P_1 \otimes P_2) \circ CNOT} = \interp{C_{CNOT} + f}$.
  \end{enumerate}
\end{proof}
\noindent
This demonstrates the construction of a ZX representation for CNOT that, while providing the correct linear map, also faithfully models the effects of any subsequent two-qubit Pauli error via a corresponding single edge flip.

Fault gadgets can be generalized to account for arbitrary weight Pauli errors.
However, the number of gadgets required to cover all non-trivial Pauli errors grows exponentially with the number of qubits.
Nonetheless, this construction establishes that, in principle, fault-accounting ZX diagrams exist for any gate, and thus, by compositionality, for any quantum circuit under circuit noise models discretized to Pauli operations.

\paragraph{Fault-Accounting Diagrams Without Fault Gadgets}

Fault gadgets, while providing a general construction for fault-accounting diagrams, can introduce significant complexity, making reasoning cumbersome.
Therefore, it is valuable to identify specific circuit compositions whose standard ZX diagram representations are already fault-accounting under circuit noise without requiring modification by gadgets.

A key example involves inputting a $\ket{+}$ state to the control of a CNOT gate.
The standard ZX diagram corresponding to this operation is fault-accounting under circuit noise:

\begin{proposition}
  \label{prop:CNOT-plus-state}
  Let $C$ be the circuit consisting of preparing the first qubit in $\ket{+}$ followed by a CNOT gate controlled by the first qubit.
  Let $N_{Pauli_2}$ be the noise model where any two-qubit Pauli error may occur immediately after the CNOT gate.
  Then the diagram $\mathcal{M}_{std}(C)$ shown below is fault-accounting for $C$ under $N_{Pauli_2}$.
  \[
    C\quad=\quad \tikzfig{03-errors/fault-accounting/cnot-plus-state}
    \qquad\qquad\qquad\qquad
    \mathcal{M}_{std}(C)\quad=\quad \tikzfig{03-errors/fault-accounting/fault-accounting-cnot-plus-state}
  \]
\end{proposition}
\begin{proof}
  For each fault $f$ previously unaccounted for by $\mathcal{M}_{std}(CNOT)$, there is now a corresponding single edge flip $(e_f, t_f)$ in $D$ that produces the required effect $\interp{C+f}$:
  \[
    \tikzfig{03-errors/fault-accounting/cnot-plus-state-proof}
  \]
\end{proof}

\begin{proposition}
  \label{prop:CNOT-plus-measurement}
  Let $C$ be the circuit consisting of a CNOT followed by a Z-basis measurement on the second qubit.
  Let $N_{Pauli_2}$ be the noise model where any two-qubit Pauli error may occur immediately after the CNOT gate.
  Then the diagram $\mathcal{M}_{std}(C)$ shown below is fault-accounting for $C$ under $N_{Pauli_2}$.
  \[
    C\quad=\quad \tikzfig{03-errors/fault-accounting/cnot-measurement}
    \qquad\qquad\qquad\qquad
    \mathcal{M}_{std}(C)\quad=\quad \tikzfig{03-errors/fault-accounting/fault-accounting-cnot-measurement-simplified}
  \]
\end{proposition}
\begin{proof}
  For each fault $f$ previously unaccounted for by $\mathcal{M}_{std}(CNOT)$, there is now a corresponding single edge flip $(e_f, t_f)$ in $D$ that produces the required effect $\interp{C+f}$:
  \[
    \tikzfig{03-errors/fault-accounting/cnot-measurement-proof}
  \]
\end{proof}

\BOLDI{Another important case is when the underlying circuit is a CSS code.
In that case, for any circuit $C$ the diagram $\mathcal{M}_{std}(C)$ fault-accounting for $C$ under $N_{Pauli_2}$:}

\subsection{Detecting Errors}

For error detection within the ZX calculus, we take a circuit-centric perspective, similar to \textcite{delfosseSpacetimeCodes2023,townsend-teagueFloquetifyingColourCode2023}, utilising Pauli webs and, specifically, detecting regions.
The core principle relies on parity measurements associated with these regions.
For an ideal diagram, the expected parity of measurement outcomes within a detecting region is fixed by the parity of elements that anticommute with the region's effective check; see \autoref{thm:detecting-region}.

A fault $\mathcal{F}$ is detected if it flips this expected parity.
This occurs if and only if the combined Pauli operator corresponding to $\mathcal{F}$ anticommutes with the effective check operator of a detecting region.
This motivates the following definitions:
\begin{definition}[Detectability of Faults]
  \label{def:detectability}
  The fault $\mathcal{F}$ is \emph{detectable} if there exists a detecting region in $D$ that has an odd overlap\BOLDI{Define odd overlap} with $\mathcal{F}$.
  Otherwise, $\mathcal{F}$ is \emph{undetectable}.
\end{definition}

The robustness of a diagram against undetectable logical errors is quantified by its distance:
\begin{definition}[ZX distance]
  \label{def:zx-dist}
  Given a ZX diagram $D$, its \emph{ZX distance} $d$ is the minimum weight $wt(\mathcal{F})$ of any fault $\mathcal{F}$ that is both non-trivial and undetectable:
  \[ d = \min \{ wt(\mathcal{F}) \mid \interp{D + \mathcal{F}} \not= \interp{D} \land \mathcal{F} \text{ is undetectable } \} \]
\end{definition}
\noindent
The ZX distance is trivial ($d=1$) for diagrams with noisy boundaries, as single edge flips on boundary wires cannot be detectable by internal detecting regions.
Non-trivial distance ($d > 1$) can be achieved in closed ZX diagrams or those with protected (idealized) boundaries.

The ZX distance directly determines the error correction capability, mirroring the standard result in quantum error correction:
\begin{theorem}
  \label{thm:correcting-circuits}
  Given a ZX diagram $D$ with ZX distance $d$, it is possible to correct any fault $\mathcal{F}$ with weight $wt(\mathcal{F}) \le t = \lfloor \frac{d-1}{2} \rfloor$.
\end{theorem}
\begin{proof}
  We first show that any two distinct faults $\mathcal{F}_1, \mathcal{F}_2$ with weight $w_1, w_2 \le t$ must produce different syndromes, up to equivalence by trivial faults (those satisfying $\interp{D+\mathcal{F}_{trivial}}=\interp{D}$).
  Assume, for contradiction, that $\mathcal{F}_1 \not\equiv \mathcal{F}_2$ have the same syndrome.
  Then $\mathcal{F} = \mathcal{F}_1 \times \mathcal{F}_2$ is a fault with weight $wt(\mathcal{F})$ at most $w_1 + w_2 \le 2t \le d-1$.
  Since $\mathcal{F}_1$ and $\mathcal{F}_2$ have the same syndrome, their combination $\mathcal{F}$ must have no syndrom and, thus, be undetectable.
  By definition of distance, any undetectable fault with weight less than $d$ must be trivial --- it is spacetime stabilized.
  Thus, $\mathcal{F}$ must be a trivial fault.
  This implies that $\mathcal{F}_1$ and $\mathcal{F}_2$ must be equivalent up to spacetime stabilizers of the circuit.
  Therefore, any fault with weight $w \le t$ has a unique syndrome up to spacetime equivalence.

  Upon measuring the syndrome, the unique equivalence class of faults is identified.
  Standard decoding procedures can determine the most likely representative fault in this class and the appropriate correction.
  Applying the correction removes the error, up to a trivial fault, thus correcting the computation.
\end{proof}


\subsection{Equivalence in a Faulty Setting}

Standard equivalence between ZX diagrams or quantum circuits is insufficient when considering noise, as linearly equivalent diagrams can exhibit different resilience to faults.
This necessitates a stronger notion, \emph{fault equivalence}, which ensures that undetectable faults in equivalent diagrams yield the same robustness to noise:

\begin{definition}[$d$-fault-equivalence and fault equivalence]
\label{def:fault-equivalence}
  Two ZX diagrams $D_1$ and $D_2$ satisfying $\interp{D_1} = \interp{D_2}$ are \emph{$d$-fault-equivalent} if for all faults $\mathcal{F}_1$ on $D_1$ with weight $wt(\mathcal{F}_1) < d$, we have either:
  \begin{enumerate}
    \item $\mathcal{F}_1$ is detectable, or
    \item there exists a fault $\mathcal{F}_2$ on $D_2$ such that:
    \begin{itemize}
      \item $wt(\mathcal{F}_2) \leq wt(\mathcal{F}_1)$ and
      \item $\interp{D_1 + \mathcal{F}_1} = \interp{D_2 + \mathcal{F}_2}$.
    \end{itemize}
  \end{enumerate}
  The condition must also hold symmetrically for all faults $\mathcal{F}_2$ on $D_2$ with weight $wt(\mathcal{F}_2) < d$.
  $D_1$ and $D_2$ are fault-equivalent if they are $d$-fault-equivalent for all $d \in \mathbb{N}$.
\end{definition}

Intuitively, $d$-fault-equivalence guarantees a symmetric relationship between the undetectable faults (of weight less than $d$) in two diagrams.
This ensures that one diagram cannot achieve a specific undetectable fault on the data qubits with \enquote{less noise} than the other.

%We can view the set of all possible, undetectable faults $\{\mathcal{F}_1, ..., \mathcal{F}_n \}$ of weight at most $d$ on some diagram $D$ to give rise to a set of linear maps $S_d = \{\interp{D + \mathcal{F}_1}, ..., \interp{D + \mathcal{F}_n}\}$.
%Intuitively, we can view these sets of linear maps for each $d \in \mathbb N$ as deviations from the ideal linear map if at most $d$ edge flips occur.
%The linear maps in each set determine ``how far you can strive'' from the ideal map within $d$ many edge flips.

This distinction is critical.
Consider the direct implementation of a weight-four Pauli Z measurement versus its linearly equivalent CNOT-based implementation:
\[
  \tikzfig{03-errors/naive-rewrite}
\]
These diagrams are not fault-equivalent.
As shown below, a single edge flip on the auxiliary wire in the CNOT-based implementation propagates to induce a weight-two logical Pauli error on the data qubits:
\[
  \tikzfig{03-errors/naive-rewrite-error}
\]
Since the above fault has no equivalent in the direct implementation, the condition of \autoref{def:fault-equivalence} is violated, and therefore the two diagrams are not $2$-fault-equivalent.

Substituting diagrams based only on linear equivalence, without ensuring fault equivalence, can inadvertently decrease the overall ZX distance of a larger diagrammatic context.
Techniques such as the use of idealized edges or employing \emph{fault-aware} ZX rewrite rules (\autoref{subsec:rewrites}) are necessary to ensure that diagram transformations produce fault-equivalent diagrams and, consequently, do not inadvertently reduce the encoded robustness against noise.

\paragraph{Hardness of Deciding Fault Equivalence}
Checking whether two quantum circuits or ZX diagrams are fault-equivalent is computationally hard.
We establish this by relating the problem to the known hardness of computing the distance of stabilizer codes~\parencite{7097029}, showing that checking fault equivalence is at least \#P-hard.

First, we establish a connection between fault equivalence and the ZX distance:
\begin{proposition}
  \label{prop:dist-as-fault-equivalence}
  Let $D$ be a ZX diagram with ZX distance $d$.
  Let $D_{ideal}$ be the corresponding fault-free diagram where all edges are replaced by idealized edges.
  Then $D$ is $d'$-fault-equivalent to $D_{ideal}$ if and only if $d' \leq d$.
\end{proposition}
\begin{proof}
  By \autoref{def:fault-equivalence}, $D$ is $d'$-fault-equivalent to $D_{ideal}$ iff for every fault $\mathcal{F}$ on $D$ with weight $wt(\mathcal{F}) < d'$, either $\mathcal{F}$ is detectable, or there exists a fault $\mathcal{F}_{ideal}$ on $D_{ideal}$ with $wt(\mathcal{F}_{ideal}) \le wt(\mathcal{F})$ and $\interp{D+\mathcal{F}} = \interp{D_{ideal}+\mathcal{F}_{ideal}}$.
  The only possible fault in $D_{ideal}$ is the empty fault $\mathcal{F}_{\emptyset}$.
  Thus, the second condition requires $\mathcal{F}$ to satisfy $\interp{D+\mathcal{F}} = \interp{D_{ideal}+\mathcal{F}_{\emptyset}} = \interp{D_{ideal}} = \interp{D}$, meaning that $\mathcal{F}$ must be a trivial fault.
  Therefore, $D$ is $d'$-fault-equivalent to $D_{ideal}$ if and only if all faults $\mathcal{F}$ on $D$ with weight $wt(\mathcal{F}) < d'$ are either detectable or trivial.
  This condition holds precisely when $d' \leq d$.
\end{proof}
\noindent
This proposition establishes that determining the ZX distance $d$ is reducible to checking $d'$-fault-equivalence against an idealized diagram.
We use this to show the hardness of deciding fault equivalence in general.

\begin{corollary}
  Deciding $d$-fault-equivalence between two ZX diagrams is at least \#P-hard.
\end{corollary}
\begin{proof}
  Consider a quantum stabilizer code defined by $S = \{S_1, \dots, S_m\}$ with code distance $d_{code}$.
  Construct a ZX diagram $D$ representing the process of performing an ideal measurement of all stabilizers in $S$, allowing a fault $\mathcal{F}$ to occur, and then performing another ideal measurement of all stabilizers in $S$.
  Graphically this is depicted as follows:
  \[
    D\ \ =\ \ \tikzfig{03-errors/ft-equiv-NP-hard}
  \]
  An undetectable fault $\mathcal{F}$ in $D$ corresponds to a logical operator of the code; the minimum weight of such a fault is $d_{code}$.
  Therefore, the ZX distance $d_{Z\!X}$ of $D$ diagram equals the code distance $d_{code}$.
  By \autoref{prop:dist-as-fault-equivalence}, checking if $D$ is $d'$-fault-equivalent to its idealized version $D_{ideal}$ is equivalent to determining if the ZX distance $d_{Z\!X}$ is less then $d'$.
  Thus, calculating the ZX distance $d_{Z\!X} (= d_{code})$ can be solved by checking $d'$-fault-equivalence for different $d'$.
  Since determining $d_{code}$ is \#P-complete~\parencite{7097029}, checking $d'$-fault-equivalence must be at least \#P-hard.
  \textcolor{red}{This is wrong: decoding is \#P-hard. Calculating distance might not be}
\end{proof}


==> sections/old/04-fault-tolerance.tex <==
\section{A Unified Perspective of Noise Resilience with Fault Equivalence}
\label{sec:FTQC}

Fault equivalence constitutes the foundational notion of this work.
In this section, we employ it to both to recover standard notions from the literature on quantum error correction and fault tolerance, and to formulate our new definition of fault tolerance.

\subsection{Quantum Error Correction as Fault Equivalence}

Standard definitions of quantum error correction relate the code's distance to its ability to detect or correct errors.
Focusing on error detection, a common definition is:

\begin{definition}[Quantum Error Detection (Standard Definition)]
\label{def:qec-lit}
A linear map $enc: \mathbb C^{2^k} \to \mathbb C^{2^n}$ is an encoder for a \emph{quantum error-detecting code} with distance $d$ if there exists a linear map $dec: \mathbb C^{2^n} \to \mathbb C^{2^k}$ (the decoder) such that for all faults $\mathcal{F}$ with weight $wt(\mathcal{F}) < d$ applied to the encoded state, the fault $\mathcal{F}$ is detectable by the decoder.
% \tikzfig{04-fault-tolerance/def-qec}
\end{definition}

This concept can be expressed directly using fault equivalence:

\begin{definition}[Quantum Error Detection (Fault Equivalence)]
\label{def:qec}
An encoding $enc: \mathbb{C}^{2^k} \to \mathbb{C}^{2^n}$ corresponds to a distance $d$ quantum error-detecting code if there exists a decoder $dec: \mathbb{C}^{2^n} \to \mathbb{C}^{2^k}$ such that:
\[\tikzfig{04-fault-tolerance/def-qec-dist-preserv}\]
\end{definition}

Here, the universal quantification over all detectable faults of weight less than $d$ in \autoref{def:qec-lit} is absorbed into the $d$-fault-equivalence.
The fault-equivalence condition requires that any fault of weight less than $d$ on the right-hand side has to either be detectable or has to have an equivalent faults on the left-hand side.
As the left-hand side is idealized as fault-free the only fault it allows is the trivial, empty fault.
This means that any fault of weight less than $d$ either has to be detectable or has to be equivalent to the trivial error.
This is exactly the usual definition about the detectability of faults.

%Before turning our attention to fault-tolerant circuit synthesis, we have to define what we mean by fault tolerance.
%In this section, we give a definition of fault-tolerant quantum computing in terms of $d$-fault-equivalence of ZX diagrams.
%We give a solution to achieving fault tolerance via a gadget-based protocol that creates similar circuits to the protocol proposed by \textcite{gottesmanSurvivingQuantum2024}.

\subsection{Fault Tolerance as Fault Equivalence}

Quantum Error Correction (QEC) is primarily about protecting quantum data (states) from noise by encoding it with redundancy such that errors can be detected and corrected.
Similarly, fault-tolerant quantum computing aims to protect quantum computations (circuits) from faults such that errors can be detected and corrected.

We define:
\begin{definition}[Fault-tolerant quantum computation under adversarial noise]
    Given an ideal quantum circuit $C$, a circuit $C_{FT}$ is a \emph{$d$-fault-tolerant implementation} of $C$ under adversarial noise if there exists a fault-accounting ZX diagram $FT$ for $C_{FT}$ such that:
    \[
        \tikzfig{04-fault-tolerance/def-fault-tolerance}
    \]
\end{definition}

That is, given an idealized quantum circuit $C$ that we want to execute, we have to find an encoding of that circuit $C_{FT}$ that performs the same computation with redundancy in such a way that faults can be detected and corrected.
By requiring that the fault-accounting ZX diagram of $C_{FT}$ is $d$-fault-equivalent to the idealized, fault-free ZX diagram $D$ of $C$, we require that any fault in $C_{FT}$ of weight less than $d$ must either be detectable or has to have a corresponding fault in $D$.
However, as we idealize $D$ to allow no faults, it must be detectable.
Thus, we have encoded $C$ in such a way that fault of weight less than $d$ must be detectable and therefore, by \autoref{thm:correcting-circuits}, faults of weight at most $\lfloor \frac{d-1}{2} \rfloor$ must be correctable.

Note that, as we idealize $D$ to be fault-free it does not matter what kind of mapping we use from $C$ to $D$, as long as $C$ and $D$ represent the same linear map.

%We have therefore utilized the ZX calculus and fault equivalence to provide a formal definition of fault-tolerant implementations.
%We could have instead defined similar notions of behaviour and equivalence in a faulty setting on quantum circuits directly, skipping the ZX calculus entirely.
%However, while the ZX calculus might not seem essential at this point, we will make increasing use of its ability to specify, synthesise and optimise quantum circuits.
%Thus, without the ZX calculus many of the observations to come, especially in \autoref{sec:fault-tolerant-syndrome-extraction}, would be a lot less obvious.


\begin{remark}[Adversarial vs\@. Stochastic Noise]
    An important limitation of this definition is that it is for fault-tolerant quantum computation \emph{under adversarial noise}.
    In physical systems, noise is often stochastic, occurring randomly over time.
    Under stochastic noise, the timing of fault detection and correction matters significantly, as uncorrected faults can accumulate.
    A circuit performing frequent checks might behave better stochastically than one with the same adversarial distance $d$ that only checks at the end.
    However, performance under adversarial noise is typically a good indicator for performance under stochastic noise, especially when analyzing local circuit components.
    For the purposes of this paper, as we focus on relatively small, individual gadgets, we work under adversarial noise and leave stochastic noise as future work.
\end{remark}

While we provide fault-aware rewrites that provably preserve fault equivalence in \autoref{sec:ft-circuit-synthesis}, synthesizing a fault-tolerant circuit remains a difficult task.
One way to approach it is via more structured protocols for fault-tolerant quantum computation.
Existing FTQC methodologies, such as lattice surgery~\parencite{debeaudrapZXCalculus2020} or Gottesman's gadget-based fault-tolerant protocol~\parencite{gottesmanSurvivingQuantum2024}, can be viewed within our framework.
They provide systematic methods for transforming an ideal logical circuit diagram into a protected implementation.
For example, in lattice surgery each logical wire is expanded into a $d$-fault-equivalent, $d\times d$-sized patch of the surface code and all the boxes broken into more elementary operations~\parencite{debeaudrapZXCalculus2020} for which we can find $d$-fault-equivalent implementations.

\subsection{Gadget-Based Fault Tolerance using Fault Equivalence}

Gadget-based fault-tolerant protocols construct fault-tolerant implementations of ideal logical circuits by replacing logical operations by fault-tolerant gadgets.
For the remainder of this section, we formalize a gadget-based protocol in terms of $d$-fault-equivalence with slightly more permissive criteria than those of \textcite{gottesmanSurvivingQuantum2024}.

Closely mirroring the definition of \textcite{gottesmanSurvivingQuantum2024}, we can use an error-correcting code to define a gadget-based fault-tolerance protocol as:
\begin{definition}[Gadget-based fault-tolerant protocol]
    A \emph{gadget-based fault-tolerant protocol} is defined relative to a distance $d$ QEC code ($enc, dec$) along with the following fault-tolerant gadgets:
    \begin{itemize}
        \item Gate gadgets
        \begin{itemize}
            \item State preparation gadget for at least one type of state
            \item Measurement gadget for at least one type of measurement
            \item Gate gadget for a universal gate set
        \end{itemize}
        \item Error correction gadget
    \end{itemize}
\end{definition}

The goal is to replace all the gates by their fault-tolerant gadgets interlaced with error correction gadgets to get the encoded, fault-tolerant circuit.
Thus, each of these gadgets has to satisfy certain behavioural requirements in a faulty setting.

%Gadget-based fault-tolerant protocols are defined with respect to a quantum error correction code $enc$, for which we know that there exists a decoder such that:
%\[\tikzfig{04-fault-tolerance/def-qec-dist-preserv}\]

We can view a quantum error correction code as encoding the trivial computation, i.e.\@ idling.
However, in an actual computation, we want to be able to perform operations.
But performing computations on encoded data might spread errors unfavourably or introduce new ones.
Therefore, gadgets that perform a computation on encoded data have to satisfy certain constraints.
For example, consider some operation $g_1$ on one code block of $k$ logical qubits.
We say, $\overline{g_1}$ is a fault-tolerant gadget for $g_1$, if it satisfies the following $d$-fault-equivalence:
\[\tikzfig{04-fault-tolerance/def-ft-gadget-single-qubit}\]

Applying the $d$-fault-equivalence definition:
any fault within the composed diagram must either be detectable or correspond to a fault within the ideal logical gate diagram.
As an ideal gate permits only the trivial fault, any undetectable fault $\mathcal{F}$ in the implementation with $wt(\mathcal{F}) < d$ must result in the correct logical operation.
This ensures low-weight faults do not cause logical errors.

More generally, we can define:
\begin{definition}[$d$-Fault-Tolerant Gadget Implementation]
    \label{def:fault-tolerance}
    Given a quantum error correction code $enc: \mathbb{C}^{2^k} \to \mathbb{C}^{2^n}$ with its ideal decoder $dec: \mathbb{C}^{2^n} \to \mathbb{C}^{2^k}$ and a logical operation $g: (\mathbb{C}^{2^k})^{m_i} \to (\mathbb{C}^{2^k})^{m_o}$ from $m_i \in \mathbb{N}$ input code blocks to $m_o \in \mathbb{N}$ output code blocks, a $d$-fault-tolerant implementation of $g$ is a quantum circuit $C_{\overline{g}}: (\mathbb{C}^{2^n})^{m_i} \to (\mathbb{C}^{2^n})^{m_o}$ such that there exists a ZX diagram $\overline{g}$ that is fault-accounting for $C_{\overline{g}}$ and satisfies the following $d$-fault-equivalence condition:
    \[\tikzfig{04-fault-tolerance/def-ft-gadget}\]
\end{definition}
\noindent
For $m_i = m_o = 1$ and $g = id$, we are left with a single encoder followed by the ideal decoder which trivially holds by the properties of the quantum error correction code.

More generally, though, our definition of a fault-tolerant gadget captures substantially more cases.
In particular, having given it for an arbitrary number of input and output code blocks, this definition encapsulates many special cases we might be interested in.
For example, for a universal gate set consisting of operations of weight one and two, we need to find fault-tolerant gadgets satisfying the conditions depicted below:
\begin{align*}
    \text{\small State: } \quad \resizebox{0.28\columnwidth}{!}{\tikzfig{04-fault-tolerance/def-ft-gadget-state-prep}} && \text{\small Single-qubit gate: } \quad \resizebox{0.35\columnwidth}{!}{\tikzfig{04-fault-tolerance/def-ft-gadget-single-qubit}}\\
    \text{\small Measurement: } \quad \resizebox{0.28\columnwidth}{!}{\tikzfig{04-fault-tolerance/def-ft-gadget-measurement}} && \text{\small Two-qubit gate: } \quad \resizebox{0.35\columnwidth}{!}{\tikzfig{04-fault-tolerance/def-ft-gadget-two-qubit}}\\
\end{align*}

Assuming that we have found such fault-tolerant implementations for all the operations we want to perform, we can replace the individual gates in our original, idealized circuit.
For the sake of simplicity, we assume that the code of our choice encodes one logical qubit per code block, i.e.\@ $k = 1$.
This replacement yields a diagram $d$-fault-equivalent to the original ideal circuit diagram:
\begin{center}
    \resizebox{\columnwidth}{!}{
         \tikzfig{04-fault-tolerance/ft-ideal-circuit} $\underset{\tiny fault-d}{=}$ \tikzfig{04-fault-tolerance/dist-rewrite-ideal-circuit}}
\end{center}
\noindent
This rewritten structure, composed of FT gate gadgets, forms the core of the implementation.
However, standard protocols interleave these with explicit fault-tolerant error correction steps.

The final necessary component is the fault-tolerant error correction gadget:
\begin{definition}[Fault-tolerant error correction]
    \label{def:ftec}
    Given a quantum error correction code $enc: \mathbb{C}^{2^k} \to \mathbb{C}^{2^n}$ with distance $d$, a fault-tolerant error correction gadget is a quantum circuit $C_{FTEC}: \mathbb{C}^{2^n} \to \mathbb{C}^{2^n}$ such that there exists a ZX diagram $FTEC$ that is fault-accounting for $C_{FTEC}$ and satisfies the following condition:
    \[\tikzfig{04-fault-tolerance/def-ftec}\]
\end{definition}
\noindent
Using this final gadget, we get the full structure:
\[\tikzfig{04-fault-tolerance/rewriting-circuit-final}\]

Thus, if we have quantum circuits that fault-tolerantly implement each of these gadgets, we have our encoded fault-tolerant circuit.
In particular, we are guaranteed that any combination of faults in the circuit corresponds to at most as many edge flips in the corresponding ZX diagram.
As this ZX diagram is defined to be $d$-fault-equivalent to the idealized fault-free diagram, any combination of less than $d$ faults must be detectable, achieving a $d$-fault-tolerant implementation of the circuit.

Readers familiar with Gottesman's gadget-based fault-tolerance protocol might recognise the extended rectangles~\parencite{gottesmanSurvivingQuantum2024}.
However, to fully show the relationship of our protocol to Gottesman's, we have to relate the respective fault-tolerance conditions for the gadgets which we will do, amongst other things, in the following section.


==> sections/old/05-ft-circuit-synthesis.tex <==
\iffalse
  \section{Fault-tolerant circuit synthesis}
  \label{sec:ft-circuit-synthesis}
  Given our specification of fault-tolerant gadgets, we can now turn our attention towards fault-tolerant circuit synthesis, i.e.\@ coming up with quantum circuits that fault-tolerantly implement our gadgets.
  To simplify the problem, we can break it into two steps:
  \begin{enumerate}
    \item Identifying the linear map we want to perform which we call the \emph{specification}
    \item Finding a quantum circuit that fault-tolerantly implements that specification
  \end{enumerate}

  For example, if we have some quantum error correction code $enc$ and a logical operation $g$, we want to implement.
  Then, in the first step, we can identify a linear map $S_{\overline{g}}$ that, if perfectly executed, satisfied our fault-tolerance conditions, i.e.:
  \[\tikzfig{05-ft-synthesis/ft-specification}\]
  Once we have identified the \emph{specification}, the second challenge is to find a quantum circuit $C_{\overline{g}}$ that fault-tolerantly implements that specification, i.e.\@ a quantum circuit for which there exists a fault-accounting ZX diagram ${\overline{g}}$ that is $d$-fault-equivalent to $S_{\overline{g}}$:
  \[\tikzfig{05-ft-synthesis/implementing-specification}\]
  Implementing a specification is the requirement that any fault $\mathcal F$ during $C_{\overline{g}}$ is either detectable or corresponds to at most $|\mathcal F|$ errors on the inputs and outputs of $C_{\overline{g}}$, i.e.\@ does not propagate out to become a larger fault.


  \subsection{Finding specifications}
  Finding a specification for a linear map can be challenging.
  A particular challenge created by our definition above is that the decoder, solving an NP-hard problem, is difficult to reason about.
  Therefore, we will provide sufficient conditions for a specification that are easier to verify.
  In fact, with some minor assumptions on the decoding process, these sufficient conditions are formally equivalent to the fault-tolerance conditions provided by \textcite{gottesmanSurvivingQuantum2024}.

  \subsubsection{Fault-tolerant state preparation}
  Usually, fault-tolerant state preparation is defined as preparing the encoding of the logical state in such a way that any fault $\mathcal F$ during the preparation is either detected or creates at most $|\mathcal F|$ many data errors \textcolor{green}{(cite)}.
  We will give an alternative, equivalent definition:
  \begin{definition}
    \label{def:ft-condition-state}
    Given a quantum error correction code $enc: \mathbb{C}^{2^k} \to \mathbb{C}^{2^n}$ with distance $d$ and a logical state $\psi \in \mathbb{C}^{2^k}$, a specification $S_{\overline{\psi}} \in \mathbb{C}^{2^n}$ is \emph{correct for $\psi$} if:
    \begin{gather}
      \tag{correctness}\label{state-correctness}\refstepcounter{equation}
      \tikzfig{05-ft-synthesis/def-state-correctness}
    \end{gather}
  \end{definition}

  \begin{proposition}
    \label{prop:ft-state-prep}
    Let $S_{\overline{\psi}}$ be a specification for some logical state $\psi \in \mathbb{C}^{2^k}$.
    Then a quantum circuit $C_{\overline{\psi}}$ for which there exists a fault-accounting ZX diagram $\overline{{\psi}}$ that implements $S_{\overline{\psi}}$ satisfies the fault-tolerance conditions outlined in \autoref{def:fault-tolerance}.
  \end{proposition}
  \begin{proof}
    We have:
    \[\tikzfig{05-ft-synthesis/state-ft-proof}\]
    Thus, $\overline{{\psi}}$, which is fault-accounting for $C_{\overline{{\psi}}}$ satisfies the fault-tolerance condition given in \autoref{def:fault-tolerance}.
  \end{proof}
  As such, we have proven that this condition is sufficient for a state preparation to be fault-tolerant according to \autoref{def:fault-tolerance}.
  More generally, this condition is equivalent to the usual definition of state preparation: the fact that the circuit should prepare the encoding of the logical state is guaranteed by the specification and the fact that any fault $\mathcal F$ during the preparation is either detected or creates at most $|\mathcal F|$ data errors is guaranteed by $\overline{{\psi}}$ being an implementation of $S$.
  Similarly, relating it to \textcite{gottesmanSurvivingQuantum2024}, we can state:
  \begin{proposition}
    Then a quantum circuit $C_{\overline{\psi}}$ performs fault-tolerant state preparation according to \autoref{prop:ft-state-prep} if and only if
    \begin{itemize}
      \item It is fault-tolerant according to \textcite{gottesmanSurvivingQuantum2024}
      \item All errors it detects are immediately corrected
    \end{itemize}
  \end{proposition}
  \begin{proof}
    See \autoref{apepndix}
  \end{proof}
  \textcolor{green}{TODO: move up ZX distance preservation (possibly change definition of distance), then we can make this slightly more understandable}
  One major difference between Gottesman's definition and ours is that we allow errors that propagate badly, as long as they are detected.
  Many state preparation protocols would simply repeat-until-success.
  However, this is not necessary.
  As we have additional information about the existence of the error, we could alternatively adapt our decoder accordingly and use the faulty preparation.
  However, as long as we take the failure into account, we can still salvage the situation.
  For more details see~\autoref{appendix:error-detector-model}.

  \begin{remark}
    \label{remark:sufficient-condition}
    While this definition of fault-tolerant state preparation is sufficient, it is not necessary.
    This is due to the fact that these formulations of state preparation --- ours and Gottesman's --- count the weight of the fault.
    However, in practice, we care about how many additional faults are necessary for an logical error to occur.
    For example, in the surface code, there exists certain faults of weight two that are only as bad as faults of weight one such as $ZZ$ faults that are orthogonal to the $Z$ logical \textcolor{green}{what to cite? Maybe stack exchange?}.
    This fact is, for example, utilized in fault-tolerant syndrome extraction for the surface code utilising a syndrome extraction circuit that would in other circumstances not be fault-tolerant.
    The general definition of fault-tolerant gadgets in \autoref{sec:FTQC} takes this special case into account, talking only about the decodability of the resulting fault.
    However, the sufficient condition provided here, does not.
  \end{remark}

  To showcase an example of what a specification for fault-tolerant state preparation might look like, we can make use of prior work on reasoning about the encoders of error correction codes in the ZX calculus \textcolor{green}{(cite)}:
  \begin{example}
    \label{ex:steane-state-prep}
    A quantum circuit ${C_{\overline{\ket{0}}}}$ fault-tolerantly implements the logical state $\ket{0}$ for the Steane code, if there exists some fault-accounting ZX diagram $\overline{\ket{0}}$ for ${C_{\overline{\ket{0}}}}$ such that:
    \[\tikzfig{05-ft-synthesis/def-0-steane-code}\]
    Where, in the last step, we have replaced the $\ket{0}$ and the $enc$ by their specific ZX diagrams.
  \end{example}

  This showcases one of the many advantages of the ZX calculus as a language to talk about fault-tolerant circuit synthesis: while it is sufficiently expressive to talk about quantum circuits, it can also talk about more abstract specifications of fault-tolerant linear maps that do not directly correspond to a quantum circuits.

  \subsubsection{Fault-tolerant single-qubit gate}
  Fault-tolerant state preparation has the advantage that the sufficient condition uniquely defines a specification.
  Once we move away from state preparation, this becomes more challening.
  For logical operations on one code block, we have:
  \begin{definition}
    \label{def:ft-conditions}
    Given a quantum error correction code $enc: \mathbb{C}^{2^k} \to \mathbb{C}^{2^n}$ with distance $d$ and a logical operation $g: \mathbb{C}^{2^k} \to \mathbb{C}^{2^k}$, a specification $S_{\overline{g}}: \mathbb{C}^{2^n} \to \mathbb{C}^{2^n}$ is \emph{correct for $g$} and satisfies \emph{push-through} if it respectively:
    \begin{gather}
      \tag{correctness}\label{correctness}\refstepcounter{equation}
      \tikzfig{05-ft-synthesis/def-correctness}\\
      \tag{push-through}\label{push-through}\refstepcounter{equation}
      \tikzfig{05-ft-synthesis/def-push-through}
    \end{gather}
  \end{definition}

  While these two conditions give restrictions on valid specifications, they do not uniquely define one.
  In particular, while they define how the specification should act on the code space, they do not define how it should act outside of the code space.
  \eqref{push-through} gives restrictions on the behaviour of $S_{\overline{g}}$ outside of the code space, stating that errors before $S_{\overline{g}}$ should not be multiplied.
  However, if an error occurs before $S_{\overline{g}}$, it could, for example, either fix the error or simply propagate it to the outputs without multiplying it --- either would satisfy~\eqref{push-through}.
  This makes finding specifications for logical operations more challenging than finding specifications for state preparation.


  Once again, we can state:
  \begin{proposition}
    \label{prop:ft-logical-gate}
    Let $S_{\overline{g}}$ be a specification for some logical operation $g: \mathbb{C}^{2^k} \to \mathbb{C}^{2^k}$.
    Then a quantum circuit $C_{\overline{g}}$ for which there exists a fault-accounting ZX diagram $\overline{{g}}$ that implements $S_{\overline{g}}$ satisfies the fault-tolerance conditions outlined in \autoref{def:fault-tolerance}.
  \end{proposition}
  \begin{proof}
    We have:
    \[\tikzfig{05-ft-synthesis/proof-ft-equiv-cond-to-ft}\]
  \end{proof}

  And similarly, we can compare this definition to the one given by \textcite{gottesmanSurvivingQuantum2024}:
  \begin{proposition}
    Then a quantum circuit $C_{\overline{g}}$ performs fault-tolerantly state preparation according to \autoref{prop:ft-logical-gate} if and only if
    \begin{itemize}
      \item It is fault-tolerant according to \textcite{gottesmanSurvivingQuantum2024}
      \item All errors it detects are immediately corrected
    \end{itemize}
  \end{proposition}
  \begin{proof}
    See \autoref{appendix}
  \end{proof}

  \begin{remark}
    While we have provided sufficient conditions for state preparation and logical operations on a single code block, similar simplifying sufficient conditions for logical operations on multiple code blocks turns out to be challenging to express in terms of fault-aware rewrites as they are defined at the moment.
    In particular, for operations on multiple code blocks, we observe that a single fault before the operation is allowed to spread to become a single fault on each of the output code blocks --- this is still fault-tolerant as any one of them still requires at least $d - 1$ additional faults to have a logical error.
    However, this push-through is not a fault-equivalence relationship, as a single fault is multiplied to become one fault per code block thereby multiplying the weight of the fault.
    This comes down to a similar observation as previously made in \autoref{remark:sufficient-condition} about the fact that these sufficient conditions are not necessary:
    fault-aware rewrites --- and similarly many other formalisations of fault-tolerance --- care about the weight of a fault rather than the distance to a logical error.
    This is why hook errors are challenging to reason about and similarly why we currently can not express the idea of multiplying a single fault to single faults over multiple code blocks.
    Both of these kind of faults are of relatively high weight, however, still have a large distance to a logical error.
  \end{remark}
\fi


\section{Manipulating ZX Diagrams --- Fault-aware rewrites}\label{subsec:rewrites}
\label{sec:ft-circuit-synthesis}

\subsection{Temp}

\begin{definition}{Faults locations, faults on ZX diagrams}
    Let $D$ be a ZX diagram. The fault locations of $D$ are all edges of $D$. 
    If $D$ has $k$ fault locations, then a \emph{fault} $F$ on $D$ is defined as an element in $\overline{\mathcal{P}_n}$, indicating the action of $F$ on each fault location of $D$.
\end{definition}

\begin{definition}{Edge-flip noise model}
    Let $D$ be a ZX diagram. The edge-flip noise model on $D$ consists of faults acting on at most one edge at a time. 
\end{definition}

for simplicities sake, we assume that every edge is either affected by errors of any type or no errors at all. Similar to before, we will visually indicate the noise model by drawing fault-free edges in purple. However, in contrast to the previously defined notion of noise models on quantum circuits, the edge-flip model is fully defined by the colouring of the edges of the diagram. Therefore, for the rest of this paper, we will omit additional details about the noise model on ZX diagrams. 

Given that both ZX diagrams and quantum circuits represent linear maps 

\subsection{End temp}

Fault-tolerant circuit synthesis often involves transforming or simplifying ZX diagrams that represent potentially complex implementations.
For these transformations to be useful, we need methods that preserve the relevant fault-tolerance properties, specifically $d$-fault-equivalence, not just the ideal linear map.

Even in an idealized, fault-free setting, circuit synthesis is challenging.
The ZX calculus, with its complete set of rewrite rules, offers a powerful tool.
However, standard ZX rewrites only preserve semantic equivalence, which is insufficient, as not all linearly equivalent circuits are fault-equivalent.
Applying standard rewrites carelessly can degrade fault-tolerance properties.

To overcome this, we restrict the allowed ZX rewrites to those that preserve behaviour in a faulty setting, i.e.\@ rewrites that preserve $d$-fault-equivalence.


\begin{definition}[$d$-fault-aware rewrite, fault-aware rewrite]
  \label{def:fault-tolerant-rewrites}
  A ZX rewrite $r: D_1 \to D_2$ is a \textit{$d$-fault-aware rewrite} if it preserves $d$-fault-equivalence.
  It is \textit{fault-aware} if it preserves fault-equivalence.
\end{definition}

An example, of a fault-aware rewrite is the following:

\begin{theorem}
  \label{thm:elim-rewrite}
  The following rewrite is fault-aware:
  \begin{gather}
    \tag{$r_{\text{elim}}$}\label{elim-rewrite}\refstepcounter{equation}
    \tikzfig{05-ft-synthesis/ft-rewrites/elim-rewrite}
  \end{gather}
\end{theorem}
\begin{proof}
  Any edge flip on the left diagram corresponds directly to an edge flip of the same type on either of the legs of the right diagram.
  Similarly, any combination of edge flips on the right diagram of types $P_1, P_2$ corresponds to an edge flip of type $P_1 \times P_2$ on the identity wire.
\end{proof}

A slightly more interesting fault-aware rewrite is the following:
\begin{theorem}
  \label{thm:fuse-rewrite}
  The following rewrite is fault-aware:
  \begin{gather}
    \tag{$r_{\text{fuse}}$}\label{fuse-rewrite}\refstepcounter{equation}
    \tikzfig{05-ft-synthesis/ft-rewrites/fuse-rewrite}
  \end{gather}
\end{theorem}
\begin{proof}
  \textcolor{red}{TODO: text}
  \[\tikzfig{05-ft-synthesis/ft-rewrites/fuse-rewrite-proof}\]
\end{proof}

The fault-awareness of the above rewrites are due to a  correspondance in errors.
An alternative way to achieve fault-equivalence is by introducing detecting regions to detect problematic faults.

\begin{theorem}
  \label{thm:four-legged-spider}
  The following rewrites for the four-legged spider is fault-aware:
  \begin{gather}
    \tag{$r_{4}$}\label{four-legged}\refstepcounter{equation}
    \tikzfig{05-ft-synthesis/ft-rewrites/four-legged}
  \end{gather}
\end{theorem}
\begin{proof}
  \textcolor{red}{TODO: we should be self-contained}
  Same proof as~\parencite[Theorem 3.9]{rodatzFloquetifyingStabiliser2024}
\end{proof}

Next, we mention a family of fault-aware rewrites whose preservation of fault-equivalence is slightly more complicated to prove.
\begin{restatable}{theorem}{inductiveDistRewrite}
  \label{thm:inductive-plus-dist-rewrite}
  The following rewrite for $n$-legged spiders with an even $n$ is fault-aware:
  \begin{gather}
    \tag{$r_{n^+}$}\label{n-plus-legged}\refstepcounter{equation}
    \tikzfig{05-ft-synthesis/ft-rewrites/recursive-spider}
  \end{gather}
  where the $n$-legged spider is constructed from two $\frac{n}{2}$-legged spiders and $\frac{n}{2}$ four-legged spiders.
\end{restatable}
\begin{proof}
  \textcolor{red}{TODO}
  The proof follows the same argument as~\parencite[Theorem 3.13]{rodatzFloquetifyingStabiliser2024}.
\end{proof}

Introducing idealized edges enables further fault-aware rewrites:
\begin{theorem}
  The following rewrite is fault-aware:
  \begin{gather}
    \tag{$r_{\text{perfect-elim}}$}\label{perfect-elim-rewrite}\refstepcounter{equation}
    \tikzfig{05-ft-synthesis/ft-rewrites/perfect-elim-rewrite}
  \end{gather}
\end{theorem}
\begin{proof}
  Any edge flip on the identity wire has a corresponding edge flip on the noisy wire of the right diagram.
  As the right diagram only has one noisy edge, all errors on that diagram must be edge flips of said edge.
  These correspond to edge flips on the identity.
\end{proof}

\begin{theorem}
  \label{thm:pefect-fuse-rewrite}
  The following rewrite is fault-aware:
  \begin{gather}
    \tag{$r_{\text{perfect-fuse}}$}\label{perfect-fuse-rewrite}\refstepcounter{equation}
    \tikzfig{05-ft-synthesis/ft-rewrites/perfect-fuse-rewrite}
  \end{gather}
\end{theorem}
\begin{proof}
  Since the internal edges in both diagrams are perfect, any fault $\mathcal{F}$ must occur only on the corresponding external boundary edges.
  Such faults map directly between the two diagrams with identical weight and effect, preserving $d$-fault-equivalence.
\end{proof}

A crucial property is that these rewrites can be applied locally within larger diagrams while preserving global fault equivalence:
\begin{theorem}
  \label{thm:composing-fault-tolerant-rewrites}
  Let $D$ be a ZX diagram containing a subdiagram $D_1$ in the context $D_{ctx}$.
  If $r: D_1 \to D_2$ is a $d$-fault-aware rewrite, then applying $r$ to replace $D_1$ with $D_2$ within $D$ yields a diagram $D'$ that is $d$-fault-equivalent to $D$.
  \[\tikzfig{05-ft-synthesis/prop-fault-equivalence-preservation}\]
\end{theorem}
\begin{proof}
  Consider any fault $\mathcal{F}$ affecting the diagram $D$, with weight $wt(\mathcal{F}) < d$.
  We must show that either $\mathcal{F}$ is detectable in $D$, or there exists a fault $\mathcal{F}'$ on $D'$ such that $wt(\mathcal{F}') \le wt(\mathcal{F})$ and $\interp{D+\mathcal{F}} = \interp{D'+\mathcal{F}'}$.

  If $\mathcal{F}$ is detectable in $D$, the condition is met.
  Now, assume $\mathcal{F}$ is undetectable in $D$.
  We can conceptually separate $\mathcal{F}$ into a component $\mathcal{F}_{local}$ acting entirely within the subdiagram $D_1$ and a component $\mathcal{F}_{ctx}$ acting entirely within the context $D_{ctx}$.
  Since $\mathcal{F}$ is undetectable in the full diagram $D$, its local component $\mathcal{F}_{local}$ must effectively be undetectable when considered as a fault on $D_1$.
  Because $D_1$ is $d$-fault-equivalent to $D_2$ and $wt(\mathcal{F}_{local}) \le wt(\mathcal{F}) < d$, the definition of $d$-fault-equivalence guarantees the existence of a fault $\mathcal{F}'_{local}$ acting on $D_2$ such that $wt(\mathcal{F}'_{local}) \le wt(\mathcal{F}_{local})$.

  We construct the corresponding fault $\mathcal{F}'$ on $D'$ by combining this $\mathcal{F}'_{local}$ with the original context fault $\mathcal{F}_{ctx}$.
  The total weight $wt(\mathcal{F}')$ is bounded by $wt(\mathcal{F}'_{local}) + wt(\mathcal{F}_{ctx}) \le wt(\mathcal{F}_{local}) + wt(\mathcal{F}_{ctx}) = wt(\mathcal{F})$.
  Thus, for any undetectable fault $\mathcal{F}$ on $D$ with $wt(\mathcal{F})<d$, we have constructed a suitable corresponding fault $\mathcal{F}'$ on $D'$.
  The argument holds symmetrically for faults starting on $D'$, proving that $D$ is $d$-fault-equivalent to $D'$.
\end{proof}

Since $d$-fault-equivalence is transitive, compositions of $d$-fault-aware rewrites are also $d$-fault-aware.
We can use this, to show that the expansion of the weight-four Pauli measurement using one idealized edge is fault-equivalent.
\[\tikzfig{05-ft-synthesis/ft-rewrites/naive-rewrite-dist-pres-proof}\]

==> sections/old/06-ft-error-detection.tex <==
\section{Examples: Fault-tolerant circuit extraction}
\label{sec:fault-tolerant-syndrome-extraction}

This section applies our framework to fault-tolerant syndrome extraction: the process of perfectly measuring all stabilizers of a QEC code between error events.
We first verify the correctness of Shor-style syndrome extraction~\parencite{shorFaulttolerantQuantum1996} and Steane-style syndrome extraction~\parencite{steaneActiveStabilization1997} using our framework. We then present improvements to both protocols that reduce resource overhead.

Fault-tolerant error correction typically involves three steps: (1) perfectly measuring all stabilizers, (2) classically calculating the correction, and (3) applying the correction.
The error correction protocols suggested by \textcite{shorFaulttolerantQuantum1996} and \textcite{steaneActiveStabilization1997} perform these steps separately, first executing the syndrome extraction and then classically calculating the correction.
Other error correction protocols, such as Knill-style error correction~\parencite{knillQuantumComputing2005}, break the problem up differently\BOLDI{; see \autoref{appendix:knill}}.
This section concentrates on the first step: fault-tolerant syndrome extraction.

We can use fault-equivalence to define fault-tolerant syndrome extraction:
\begin{definition}
    Let $enc$ be the encoder for a distance $d$ QEC code with stabilizer generators $S = \{S_1, \dots, S_m\}$.
    A quantum circuit $C_{SE}$ fault-tolerantly performs syndrome extraction for the code, if there exists a ZX diagram $SE$ that is fault-accounting for $C_{SE}$ and satisfies:
    \[\tikzfig{06-ft-syndrome-extraction/ideal-error-detection}\]
    where each $S_i$ is given as:
    \[
    \tikzfig{06-ft-syndrome-extraction/s-i-specification}
    \]
    potentially tensored with identity wires that the particular syndrome measurement does not act upon.
\end{definition}
Given this specification for our desired behaviour in a faulty setting, our goal is to synthesize a fault-equivalent, fault-accounting ZX diagram.

\subsection{Shor-style syndrome extraction}

Shor-style syndrome extraction~\parencite{shorFaulttolerantQuantum1996} removes fault-free edges by repeating measurements.
For example, repeating the schedule $(\lfloor \frac{d-1}{2} \rfloor + 1)^2$ times suffices~\parencite{gottesmanSurvivingQuantum2024}.
If at most $\lfloor \frac{d-1}{2} \rfloor$, i.e.\@ errors occur (a correctable number), then we can extract the correct syndrome by identifying a majority outcome across repetitions.
However, this method discard information about syndrome changes over time, focusing only on identifying $t$ iterations of the measurement schedule that are correct.

Alternatively, using our framework, we observe:
\begin{theorem}
    Let $S = [S_1, \dots, S_m]$ be the stabilizers of some stabilizer code with distance $d$. Then:
    \[\tikzfig{06-ft-syndrome-extraction/shor/claim-repeat-stabilisers}\]
    That is, repeating the measurement schedule $d$ times distance-$d$-preservingly implements the syndrome extraction.
\end{theorem}
\begin{proof}
    The proof proceeds by showing that all non-detectable internal errors (weight <d) can be pushed to the boundaries without increasing their weight.

    Since there are $d$ iterations and only consider errors of weight less than $d$, at least one iteration must be error-free.

    Consider all edge flips to the left of this error-free iteration that occurred on data wires.
    We can push these edge flips to the input wires.
    For all the measurements they anticommute with, this introduces an edge flip on the corresponding measurement wire.
    Eventually, all initial data-wire edge flips are pushed to the inputs, possibly creating additional edge flips on measurement wires.
    We can analogously push all edge flips to the right of the perfect round to the outputs.
    At this point, the total number of edge flips might have increased.
    However, the number of edge flips on the input and output wires combined is at most the weight of the original error.
    The only potential errors remaining within the $d$ repetitions are measurement errors.
    Since one round of measurements is error-free, and we assumed the error to be undetectable, all other iterations must have the same outcomes as the error-free one (otherwise, differing repeated measurements of the same stabilizer would detect an error).
For example, for low-distance codes, brute-force search can find alternatives that substantially improve on this bound~\parencite{delfosseShortShorstyle2020}.

After establishing how repetition provides fault tolerance for the overall process, we must ensure each individual stabilizer measurement is implemented fault-tolerantly.
Again, we can frame this standard problem using fault-equivalence.
The usual formulation is:
\begin{definition}[Fault-tolerant syndrome measurement]
    A quantum circuit $C$ fault-tolerantly implements a Pauli measurement if it implements the Pauli measurement such that $n$ faults are either detectable or create at most $n$ data errors and/or flip the classical outcome of the measurement.
\end{definition}

In terms of fault-equivalence, this is equivalent to:
\begin{definition}[Fault-tolerant syndrome measurement]
    A quantum circuit $C$ fault-tolerantly implements a Pauli measurement, if a ZX diagram $D$ that is fault-accounting for $C$ under circuit noise can fault-tolerantly be reduced to: 
    \[\tikzfig{06-ft-syndrome-extraction/shor/idealised-syndrome-extraction}\]
\end{definition}

One method of implementing such a measurement is offered by Shor:
\[\tikzfig{06-ft-syndrome-extraction/shor/shor-ft-proof}\]
Assuming fault-tolerant preparation of the cat state, the final ZX diagram corresponds to initializing four auxiliary qubits to the cat state, applying transversal CNOTs, and destructively measuring the auxiliary qubits.
Under this assumption, the diagram is fault-accounting for the corresponding circuit (by \autoref{prop:CNOT-plus-measurement}).
Fault-aware rewrites ensure that any set of faults $\mathcal F$ in the corresponding quantum circuit map to at most $wt(\mathcal{F})$ edge flips in the ZX diagram.
Due to the use of fault-aware rewrites these edge flips are either detectable or correspond to at most $wt(\mathcal{F})$ edge flips in the specification.
Thus, we have shown that Shor-style syndrome measurements are fault-tolerant.


\subsubsection{Fault-tolerant cat state preparation}
To implement Shor's fault-tolerant syndrome measurement, one must fault-tolerantly prepare a cat state, i.e.\@ find a quantum circuit that implements the following specification:
\[\tikzfig{06-ft-syndrome-extraction/shor/cat-state/idealised-cat-state-arbitrary}\]

This is formally equivalent to the usual notion: ``preparing the cat state such that any fault $\mathcal{F}$ is detectable or creates at most $wt(\mathcal{F})$ data errors.''
Again, a standard definition from the literature naturally translates to: ``fault-tolerantly rewrite this diagram into an executable quantum circuit.''

Using fault-aware rewrites, for weight-four cat states, we have:
\[\tikzfig{06-ft-syndrome-extraction/shor/cat-state/four-legged-derivation}\]
By \autoref{prop:CNOT-plus-measurement} and \autoref{prop:CNOT-plus-state}, this ZX diagram is fault-accounting for the corresponding cat state preparation circuit.

For $n$-legged cat states, we can first decompose the $n$-legged cat state into two $\frac{n}{2}$-legged cat states and apply this decomposition recursively:
\[\tikzfig{06-ft-syndrome-extraction/shor/cat-state/arbitrary-legged}\]
Assuming the recursive decomposition of the $\frac{n}{2}$-legged cat states is fault-tolerant, the resulting ZX diagram is fault-accounting for the corresponding circuit, making the overall circuit fault-tolerant.
\TODO{Do we need more here? This only works for cat states with $2^n$ legs. For others, we have to add extra legs first (likely there is actually something smarter as well)}

Therefore, we have shown how to prepare arbitrary cat states fault-tolerantly using this recursive construction.
Usually, cat state preparation involves designing a noise-free circuit and then adding checks to catch faults that propagate badly.
As the cat state size and fault size increase, identifying all such faults becomes exponentially harder.
In our approach, any fault is guaranteed, by construction, to be either detectable or to correspond to at most an equally sized fault in the specification (and thus at most as many data errors) – our construction is fault-tolerant by design.

\subsubsection{Alternative syndrome extraction methods}
An interesting aspect of our fault-tolerance proofs is that they do not rely on transversality, the usual argument for Shor-style methods.
This implies we can also verify non-transversal constructions.
For example, consider this alternative construction for fault-tolerant syndrome extraction:
\[\tikzfig{06-ft-syndrome-extraction/shor/shor-alternative}\]
By \autoref{prop:CNOT-plus-measurement} and \autoref{prop:CNOT-plus-state}, this ZX diagram is also fault-tolerantly equivalent to a fault-accounting diagram for its corresponding circuit, assuming fault-tolerant implementation of the cat-like linear map.
Using the construction from \textcite{rodatzFloquetifyingStabiliser2024}, we can perform this linear map for arbitrary sized cat-like linear maps:
\[\tikzfig{06-ft-syndrome-extraction/shor/cat-state/cat-like-weight-four} \qquad\qquad\qquad \tikzfig{06-ft-syndrome-extraction/shor/cat-state/cat-like-arbitrary-weight}\]


This provides an alternative fault-tolerant syndrome measurement method that is fault-equivalent to Shor-style syndrome extraction.
However, it only uses two auxiliary qubits and two measurements instead of four.
More generally, for weight $n$, it uses $\lceil \frac{n}{2} \rceil$ auxiliary qubits and measurements, compared to $n$ for the standard Shor method.

The main trade-off is that the cat state in the original Shor method can be prepared asynchronously; if errors occur during preparation, the state can be discarded and restarted.
In our new construction, the cat-like linear map gets entangled with the data qubits during its implementation, so faulty implementations cannot be simply discarded and must be handled by the outer code.
However, if the original diagram had some distance $d$, our use of fault-aware rewrites preserves fault-equivalence by \autoref{prop:dist-as-fault-equivalence}, meaning the resulting diagram still has distance $d$.
Thus, by \autoref{thm:correcting-circuits}, if overall number of errors (including those within the cat-like map) at most $\frac{d-1}{2}$, they remain correctable.


The flexibility of the ZX calculus allows generating various alternatives.
For example, one similar to \textcite{rodatzFloquetifyingStabiliser2024}:
\[\tikzfig{06-ft-syndrome-extraction/shor/shor-alternative-rodatzetal}\]
Besides being equally resource-efficient as our previous proposal, this implementation moves data qubits around the chip in a teleportation-like fashion.
This can potentially aid routing on chips with limited connectivity.

\subsection{Steane-style FTEC}
Steane proposed an alternative method for fault-tolerant error correction~\parencite{steaneActiveStabilization1997}.
Once again, the underlying question is to fault-tolerantly implement our specification: perfectly measuring all stabilizers without intermediate faults.
For Steane-style syndrome extraction, we assume the code is a CSS code, allowing separation of $X$- and $Z$-stabilizers.
For example, for the Steane code, the goal is to perfectly implement the following schedule:
\[\tikzfig{06-ft-syndrome-extraction/steane/steane-code-syndrome-measurements}\]

We can prove the correctness of Steane-style syndrome extraction using the following set of ZX rewrites:
\[\tikzfig{06-ft-syndrome-extraction/steane/steane-syndrome-extraction-steane-code}\]
The first step uses standard ZX rewrites, which are fault-aware on idealized edges.
The second and third steps are fault-aware only if the input state is stabilized by the code's stabilizers.
In this case, problematic errors that could spread unfavourably are detectable.
In particular, in the first step, problematic errors are $Y$ errors between the two measurement blocks.
However, if fewer than $d$ such errors occur, the properties of the code ensure they are detectable.
Similarly, in the second rewrite, problematic errors correspond to measurement errors, which are detectable if fewer than $d$ occur.
Finally, we can use the fault-aware rewrites (identity) and (unfuse) to complete the proof.

The resulting circuit can be read as preparing the logical $\ket{0}$ state on an auxiliary code block, transversally entangling it with the data qubits via CNOTs, and measuring the ancilla block in the $X$ basis.
Then repeating the same procedure for the $\ket{+}$ state. 

Thus, Steane-style syndrome extraction does not eliminate ideal edges through repetition like Shor's method. Instead, it transforms the problem: fault-tolerantly implementing the initial auxiliary logical states becomes the central challenge.
This is formally equivalent to solving fault-tolerant logical state preparation – again expressing an existing problem in terms of fault-aware rewrites.

\subsubsection{Fault-tolerant logical state preparation}
Fault-tolerant logical state preparation remains a challenging problem, partly due to the ideal edges involved in its specification.
For the Steane code, one distance-3-preserving preparation of the logical $\ket{0}$ state is given by \textcite{gotoMinimizingResource2016}:
\[
  \tikzfig{06-ft-syndrome-extraction/steane/ft-zero-state-steane}
  \qquad\quad\Longrightarrow\qquad\quad
  \tikzfig{06-ft-syndrome-extraction/steane/ft-zero-state-steane-in-zx}
\]

\TODO{we can probably say a little bit more here, referring back to the specification of ft-state-prep of the previous section}

\subsubsection{Fault-tolerant circuit optimization}
Similar to our improvements to Shor-style syndrome extraction, we can also bend around some of the legs of the logical state preparation component within the Steane extraction circuit:
\begin{align*}
    \tikzfig{06-ft-syndrome-extraction/steane/floquetify-steane-syndrome-extraction-1}&\\
    \tikzfig{06-ft-syndrome-extraction/steane/floquetify-steane-syndrome-extraction-2}&\\
    \tikzfig{06-ft-syndrome-extraction/steane/floquetify-steane-syndrome-extraction-3}&
\end{align*}
This yields a circuit that formally performs the same action as Steane-style syndrome extraction but uses fewer auxiliary qubits and gates.
Just as above, we have traded the problem of fault-tolerant state preparation for fault-tolerantly implementing a corresponding linear map.
This trades the ability to asynchronously prepare the states for executing linear maps that are more efficient to prepare.
While general results on efficiency gains are not presented here, this specific example for the Steane code demonstrates the potential of this construction, reducing the number of auxiliary qubits from eight to five and the number of CNOTs used outside the transversal CNOT block from 11 to eight.

\TODO{qubit gains: half the number + whatever we need for preparation vs logical map}

==> sections/old/07-conclusion.tex <==
\section{Conclusion}
provided formal definitions of quantum error correction code, fault-tolerance, cat-state-prep and error-detection in terms of distance-preserving rewrites
